Knowing When to Stop: Efficient Context Processing via Latent Sufficiency Signals

Large language models (LLMs) process entire input contexts indiscriminately, which is inefficient when the information required to answer a query is localized within the context. We present dynamic context cutoff, a novel method enabling LLMs to self-terminate processing upon acquiring sufficient task-relevant information. Through analysis of model internals, we discover that specific attention heads inherently encode "sufficiency signals" -- detectable through lightweight classifiers -- that predict when critical information has been processed. This reveals a new efficiency paradigm: models' internal understanding naturally dictates processing needs rather than external compression heuristics. Comprehensive experiments across six QA datasets (up to 40K tokens) with three model families (LLaMA/Qwen/Mistral, 1B-70B) demonstrate 3.4% accuracy improvement while achieving 1.33x token reduction on average. Furthermore, our method demonstrates superior performance compared to other context efficiency methods at equivalent token reduction rates. Additionally, we observe an emergent scaling phenomenon: while smaller models require probing for sufficiency detection, larger models exhibit intrinsic self-assessment capabilities through prompting.

==> sections/discussion.tex <==
\section{Analysis}
In this section, we conduct a series of investigations to better understand our method. We focus on the short-form dataset and mainly use LLaMA3.2-1B model for our analysis. 


\noindent\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{-2mm}
\includegraphics[width=\linewidth]{figures/p90_metrics.png}
\vspace{-2mm}
\captionof{figure}{F1 score and Recall at 90\% precision for sufficiency detection. Our approach reliably identifies when enough context is present while minimizing false positives. More results can be find in Appendix \ref{app:recall_precision}.
}
\vspace{-5em}
\label{fig:f1_p90}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering

\centering
\vspace{-2mm}
\includegraphics[width=\linewidth]{figures/confidence_distribution.png}
\vspace{-2mm}
\captionof{figure}{Confidence progression across context chunks. Models prediction confidence increases monotonically with more context.
}
% \vspace{mm}
\label{fig:confidence_distribution}
\end{minipage}


\subsection{Classification Threshold Analysis}
\label{sec:threshold}
The balance between the model’s prediction confidence and the classification threshold $\tau$ is a key factor in our proposed method. In Figure~\ref{fig:confidence_distribution}, we plot the model’s prediction confidence averaged over different numbers of chunks. We observe that the confidence in sufficiency predictions grows steadily as more context is processed, which indicates that useful signals are accumulating over the chunks. Consequently, once the model’s confidence exceeds $\tau$, it has likely integrated enough information. Note that stopping too early can cause information loss when critical elements of the context are excluded. 
Although F1 score is a useful measure for detecting context sufficiency, we also report Recall at high Precision to show how well our method identifies truly sufficient contexts while minimizing false positives. In Figure~\ref{fig:f1_p90}, we show results at 90\% precision and provide further findings at 95\% and 98\% precision in the appendix. This metric measures the fraction of actually sufficient contexts that are correctly identified when precision is at least 90\%. Such a metric is critical for our task as a mistaken early cutoff (false positive) can exclude relevant content and degrade the final performance. 


\noindent\begin{minipage}[t]{0.48\textwidth}
\vspace{-3em}

\subsection{Chunking and Inference Time Analysis}
\label{sec:chunking}
Chunking determines how efficiently the model processes and evaluates context sufficiency. Table~\ref{tab:chunking_strategies} compares different chunking strategies for Qwen2.5-14B. Percentage-based chunking performs consistently well, with 10\% chunking offering the best trade-off between accuracy and efficiency. While sentence-level chunking achieves the highest classification performance, it is impractical due to the increased overhead of frequent sufficiency checks.
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
    % \centering
    
    % \small
    \begin{tabular}{lccccc}
        \toprule
        \textbf{Metric} & \textbf{Sent.} & \textbf{1\%} &  \textbf{5\%} & \textbf{10\%} & \textbf{20\%} \\
        \midrule
F1-Score & 96.8 & 87.2 & 87.0 & 88.3 & 88.3 \\
R@90P & 95.4 & 90.9 & 78.4 & 85.9 & 85.8 \\
Acc. & 14.5 & 13.7 & 12.8 & 13.9 & 13.7 \\
    \bottomrule
    \end{tabular}
\captionof{table}{Sentence-level chunking achieves the highest performance but is computationally expensive. 10\% chunking offers the best balance between accuracy and efficiency.}
\label{tab:chunking_strategies}

    % \vspace{-3em}
\end{minipage}


\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/inference_time_comparison_subplots.png}
    \caption{For short contexts (1K tokens), full-context processing is faster. However, beyond 2K tokens, our method becomes more efficient, achieving faster inference when fewer than six chunks (60\% of the full context) are processed.
    }
\label{fig:inference_time_comparison_subplots}
    % \vspace{-1em}
\end{figure*}

Since these checks require processing chunks sequentially, smaller chunks lead to higher latency, as each additional step incurs computational overhead before reaching a decision even with caching. 10\% chunking is chosen to best balance the granularity and efficiency.
~\Cref{fig:inference_time_comparison_subplots} shows inference time between our method (10\% chunking) and full-context processing. For short contexts (1K tokens), directly processing the full-context is faster; however, beyond 2K tokens, our method provides great inference time savings-when fewer than six chunks (60\% of the full context) are processed. This demonstrates that our approach scales efficiently, offering increasing benefits for longer inputs.



\subsection{Universal Cutoff vs. Model-Specific Cutoff} \label{sec:future_work}
From a human perspective, each task has a ``gold'' location in the context where the final relevant information resides—once an answer is directly yielded, any further context is redundant. In such cases, a universal stopping point may be plausible. However, from a model perspective, defining a single optimal cutoff is challenging and ambiguous. For example, in in-context learning (ICL), models observe demonstration examples without a clear threshold for sufficiency. Smaller models may require more examples to generalize, while larger models may reach high confidence with fewer. This suggests a model-specific cutoff, where each model determines its own stopping threshold rather than adhering to a universal standard. This is particularly relevant in real-world applications, where different LLMs and tasks have varying context requirements. Future work could explore adaptive algorithms that learn individualized thresholds based on task structure and internal model signals. Appendix~\ref{app:model_cutoff} provides further discussion on this issue, espcially in ICL.



\section{Conclusion}
We introduce dynamic context cutoff, a method that enables LLMs to process only the minimal necessary context by detecting context sufficiency signals using model's internal representation. This approach reduces token processing by 1.33$\times$ on average while improving accuracy by 1.3\%, outperforming static methods like RAG and compression-based heuristics. We find that larger models develop emergent self-assessment capabilities, allowing them to detect sufficiency through self-prompting. By enabling models to terminate processing dynamically, our method enhances efficiency and scalability for LLM inference, paving the way for more adaptive and intelligent context processing for LLMs.


% \section*{Impact Statement}
% Our work enhance the efficiency of Large Language Models (LLMs) by enabling them to dynamically determine when sufficient information has been processed. By leveraging inherent ``sufficiency signals'' within model attention heads, our approach reduces computational costs while maintaining or even improving accuracy. This contributes to the broader goal of making LLMs more scalable and practical for real-world deployment. Beyond technical efficiency, our work has societal implications, particularly in reducing the environmental impact of large-scale inference.


==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
In this section we conduct comprehensive experiments to demonstrate the effectiveness of our method. 
\subsection{Experimental Setup}
\paragraph{Models}
We evaluate 4 open-source LLMs from different model families, ranging from 1B to 70B parameters: LLaMA3.2-1B \citep{dubey2024llama}, Ministral-8B \citep{mistral}, Qwen2.5-14B \citep{qwen2}, and LLaMA3.3-70B \citep{dubey2024llama}. Note that our proposed method is model-agnostic and can be applied to any Transformer-based LLM.


\paragraph{Datasets}
\label{sec:data}
In this work, we focus on two categories of datasets based on reasoning complexity: single-hop and multi-hop. These datasets are chosen to assess the ability of models to locate the key information across varying context structures and task.

\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{2pt}
    \setlength{\parsep}{2pt}
        \item \textbf{Single-hop Reasoning:} The answers are typically found within a single passage, requiring minimal context dependency.
\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
\setlength{\itemsep}{2pt}
\setlength{\parskip}{2pt}
\setlength{\parsep}{2pt}

        \item \textbf{SQuAD} \citep{squad}: A widely used dataset with questions based on Wikipedia passages.
        \item \textbf{Natural Questions} \citep{nq}: Contains questions derived from real-world search queries, with answers located in a single but longer passage.
        \item \textbf{Code Understanding}: We use GPT-4o to synthetically generate multiple single-function code snippets as distracor, and use the orignal PCSD \citep{pcsd} data to create a QA task dataset, requiring to first locate and then understand the relevant code. 
    \end{itemize}
    
    \item \textbf{Multi-hop Reasoning:} It requires the model to combine information from multiple parts of the context to arrive at the correct answer. Missing a single piece of information could lead to incorrect answers.
\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
\setlength{\itemsep}{2pt}
\setlength{\parskip}{2pt}
\setlength{\parsep}{2pt}
        \item \textbf{HotpotQA} \citep{yang-etal-2018-hotpotqa}: A popular dataset with multi-hop questions that require reasoning across multiple paragraphs from Wikipedia.
        \item \textbf{MUSIQUE} \citep{musique}: A dataset with compositional and nested questions that require multi-step reasoning across multiple sources.
        \item \textbf{Multi-hop Key-Value Retrieval}: A synthetic dataset designed to simulate multi-hop reasoning by requiring the exact retrieval of dependent ``key-value'' pairs. The key-value pairs are randomly generated.
    \end{itemize}
\end{itemize}

\paragraph{}
While most of these datasets are naturally short, we extend them to approximately 40K tokens to evaluate LLMs' long-context capabilities. Following approaches from \citet{lostinmiddle} and \citet{infinitybench}, we combine multiple unique documents within each dataset to create a long-form version from the original short-form datasets. We conduct experiments on both short-form and long-form (\sref{sec:context_length}). Additionally, we analyze the trade-off between inference time and context length in our method in \sref{sec:chunking}. For more details about the dataset, refer to~\Cref{app:data}. The ground-truth sufficiency cutoff for each input in the dataset is defined as the position of the \textit{last} token in the gold information span (i.e., the minimal required context for answering correctly), normalized by the total number of tokens in the input. However, this definition assumes that sufficiency is a property of the dataset rather than the model, meaning a single cutoff point applies universally across models. In reality, different models may require varying amounts of context to generate correct answers, suggesting that sufficiency could be inherently model-dependent. Investigating this distinction further is an important direction for future work and is described in more detail in \sref{sec:future_work}. 


\paragraph{Baselines}
We comprehensively evaluate our method against several existing approaches for context processing:

\begin{itemize}[leftmargin=*,noitemsep,nolistsep]
\setlength{\itemsep}{2pt}
\setlength{\parskip}{2pt}
\setlength{\parsep}{2pt}

\item \textbf{BM25} (RAG) \citep{INR-019}: A traditional retrieval algorithm ranks context chunks based on their term-frequency-based relevance to the query. The LLM processes only the top-ranked chunks.

\item \textbf{SBERT} (RAG) \citep{sbert}: Uses a transformer-based sentence encoder to compute dense vector embeddings of both queries and context chunks. Chunks are ranked by cosine similarity, improving semantic relevance over BM25.

\item \textbf{LLMLingua} (Compression) \citep{llmlingua}: 
A token-level compression approach that removes low-entropy tokens from the context based on perplexity scores from an external small language model. This reduces input length but may discard relevant information.


\item \textbf{LongLLMLingua} (Compression) \citep{longllmlingua}: An extension of LLMLingua designed for long-context scenarios. It applies a hierarchical, question-aware filtering strategy to retain critical content in multi-doc settings.

\item \textbf{LLMLingua2} (Compression) \citep{llmlingua2}: Improves over LLMLingua by explicitly learning a task-agnostic prompt compression objective. Instead of relying solely on token perplexity, it distills knowledge from a large LLM into a smaller transformer encoder, trained as a token classifier to retain essential information while compressing input.

\item \textbf{Fine-Tuned Classifier}: A small, fine-tuned model learns to predict when sufficient information has been processed. The LLM halts further input processing once the fine-tuned model classifies the current context as sufficient. More details can be found in Appendix~\ref{app:details:small_llm}.

\item \textbf{Self-Prompting}: The LLM predicts sufficiency dynamically by responding to a self-assessment prompt. See \sref{sec:self_prompt} for more details. 

\end{itemize}


\paragraph{Evaluation Metrics}
We evaluate the proposed dynamic context cutoff methods using metrics for both sufficiency classification and task performance. For sufficiency classification, we use \textbf{F1 Score}, which balances precision and recall, capturing the trade-off between false positives (overestimating sufficiency) and false negatives (underestimating sufficiency). Additionally, we report \textbf{Recall at 90\% Precision (R@90P)}, which measures the percentage of sufficient contexts correctly identified while maintaining a precision of at least 90\%. This ensures that the method reliably avoids excessive false positives while achieving high recall. For task performance, we evaluate \textbf{Accuracy}, which measures the percentage of correct task outputs (e.g., accurate answers in question answering) after context cutoff, as well as \textbf{Token Reduction}, quantifying the proportion of tokens processed relative to the full context. Following previous work \citep{helmet}, we perform model-based evaluation by using GPT-4o Mini.\footnote{gpt-4o-mini-2024-07-18} as judge to evaluate the task performance. The evaluation prompt can be found in \Cref{app:eval_prompt}.

\paragraph{Implementation Details}
The proposed dynamic context cutoff method involves three hyperparameters: the classification threshold \(\tau\), the number of attention heads used for training, and the number of classifiers in the ensemble. Among these, \(\tau\) is the key hyperparameter as it directly impacts the trade-off between efficiency and performance, as discussed in \sref{sec:threshold}. The remaining two hyperparameters are determined empirically via a standard hyperparameter sweep on the validation set, the details can be found in Appendix \Cref{app:details:classifier}.
Specifically, we set $k$ = 5 for attention heads with the highest F1 scores and train 8 lightweight classifiers for each head, selecting the top 4 with the highest AUC scores to form the ensemble. More details can be found in \Cref{app:details:dynamic_context_cutoff}. For all methods, including the proposed dynamic context cutoff method, we evaluate using percentage-based chunking with a 10\% incremental threshold, meaning each chunk contains 10\% more of the full context than the previous one. We explore different chunking strategies and inference time trade-off in \Cref{sec:chunking}. 
We use all of the datasets from both categories for probe training, refer to \Cref{app:data} for more details.


\subsection{Results}  
\label{sec:results}


\begin{figure*}[htpb!]
    \centering
    \includegraphics[width=\textwidth]{figures/accuracy_vs_reduction.png}
    \caption{Our method achieves superior efficiency-accuracy trade-offs compared to baselines. RAG degrades with scale, while Lingua2 remains competitive but lags on multihop tasks. Larger models (14B+) exhibit emergent self-awareness on context sufficiency through prompting.}
    \label{fig:accuracy_vs_reduction}
\end{figure*}



\noindent\begin{minipage}[t]{0.48\textwidth}
\paragraph{Sufficiency Classification}
Table \ref{tab:sufficiency_f1} shows that probing internal attention heads achieves superior sufficiency detection (F1 = 91.1) compared to supervised fine-tuning (79.5) and self-prompting (83.1) in 70B models, demonstrating that latent sufficiency signals are more reliable than surface-level outputs. 
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \centering
    % \small
    \vspace{-3em}
    \begin{tabular}{l c c c}
        \toprule
        \textbf{Model} & \textbf{FT} & \textbf{Prompt} & \textbf{Ours} \\
        \midrule
        LLaMA3.2-1B  & \multirow{4}{*}{79.5} & 52.6 & 88.3 \\
        Mistral-8B   &                        & 69.7 & 89.8 \\
        Qwen2.5-14B  &                        & 78.3 & 87.2 \\
        LLaMA3.3-70B &                        & 83.1 & 91.1 \\
        \bottomrule
    \end{tabular}
    \captionof{table}{Probing attention heads achieves superior F1 scores compared to supervised fine-tuning (FT) and self-prompting across all models.}
    \label{tab:sufficiency_f1}
    % \vspace{-3em}
\end{minipage}

We also observe an interesting phenomenon - while 1B models struggle with self-prompting (F1 = 52.6), 70B versions achieve much higher performance, suggesting larger models intrinsically develop self-assessment capabilities. However, our probing approach maintains consistent high performance across all model sizes, which confirms that internal activation provides the most reliable sufficiency detection regardless of model scale. 

\paragraph{Efficiency vs. Performance}
\label{sec:short_results}
Figure \ref{fig:accuracy_vs_reduction} shows the efficiency and performance trade-off between different methods. Unlike static methods (RAG and lingua family) that require predefined compression rates or top-k document selection, dynamic methods (FT, self-prompting, and our approach) adaptively determine cutoff points based on content understanding. For our proposed method, we sweep through 4 different $\tau$ values. For 1B models, our method matches RAG and LLMLingua2 in token reduction and achieves comparable accuracy. At 8B, it processes about $1.5\times$ fewer tokens with minimal accuracy drop, outperforming all baselines. For 14B+ models, the method not only reduces tokens up to $1.22\times$ but also improves accuracy.
In contrast, RAG degrades sharply with scale. FT underperforms universally, likely due to misaligned sufficiency signals across models. Interestingly, larger models (14B+) exhibit emergent self-awareness via prompting, whereas smaller models (1B-8B) perform poorly in prompting, as instruction following ability is critical for self-prompting to work effectively. The results suggest that context truncation may also mitigate the ``lost-in-the-middle'' problem, as models focus more on the end of the context, which are likely to contain key information after removal. 

\input{tables/main_results_short}
\input{tables/long_results}

\paragraph{Individual Task Performance}
\label{sec:tasks_result}
Table~\ref{tab:tasks_result} shows that our method maintains consistent performance on both single-hop tasks (49.4\% average accuracy) and multi-hop tasks (29\%), outperforming the top static baseline, LLMLingua2, by +1.5\% absolute accuracy score. In contrast, RAG methods experience a considerable drop in both settings. For a fair comparison, we report RAG results only for $k=8$, which corresponds to a compression rate of $0.8$ for lingua family or a token reduction factor of $1.25\times$. It is important to note that dynamic methods stop naturally and do not target a specific token reduction rate. Our method achieves a $1.33\times$ reduction in tokens, while the FT and Prompt methods achieve reductions of $1.54\times$ and $1.42\times$ on average, respectively. 


\paragraph{Longer Context Scenario}
\label{sec:context_length}
We evaluate our method with longer context to assess its scalability. For fair comparison, static methods are evaluated at a fixed 1.25$\times$ token reduction.  
Table \ref{tab:results_long} shows that our method consistently outperforms baselines, especially in multi-hop setting. Dynamic methods adaptively determine cutoff points, with FT achieving 1.61$\times$, Self-Prompt 1.41$\times$, and our method 1.27$\times$, ensuring minimal performance loss. Notably, RAG performs better in long-context settings, particularly for multi-hop reasoning. However, FT remains the weakest method, struggling with generalization. Self-Prompting improves with model size, as larger models better follow instructions for self-assessment. The result confirms that dynamic cutoff outperforms static heuristics. For longer context, our method provides an alternative and scalable solution for efficient inference.



==> sections/intro.tex <==
\vspace{-1em}
\section{Introduction}  
Large language models (LLMs) demonstrate remarkable capabilities across diverse tasks, yet their indiscriminate processing of entire input contexts creates inefficiencies. Standard Transformer-based architectures process every token with equal computational priority, regardless of its actual relevance to the task \citep{vaswani2017attention}. This brute-force approach creates fundamental inefficiencies: models waste computation on irrelevant context while simultaneously struggling with the ``lost-in-the-middle'' phenomenon where critical information becomes diluted in lengthy inputs \citep{lostinmiddle, RULER}. For instance, when answering a simple factual question, models process an entire document even after encountering the relevant information.


\noindent\begin{minipage}[t]{0.48\textwidth}
The human cognitive system offers an instructive contrast. When solving problems, people dynamically assess information sufficiency – we stop processing once we gather enough evidence, ignoring redundant details \citep{fiske1991social}. On the other hand, LLMs process entire contexts even after acquiring sufficient information. This raises a question: ``Can we equip LLMs with the ability to self-assess context sufficiency and terminate early without compromising accuracy?''
\\
In this work ,we present dynamic context cutoff, which enables LLMs to identify when they have acquired sufficient information for a task. 
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{figures/f1.pdf}
\vspace{-6mm}
\captionof{figure}{Our method enables language models to perform early termination by capturing sufficiency signals in key attention heads, reducing the amount of processed content while preserving performance.}
\label{fig:f1}
\end{minipage}


Our key insight emerges from the analysis of the model internals: specific attention heads in transformer layers exhibit strong sensitivity to information sufficiency (\sref{sec:probing_sufficiency}). By monitoring these ``indicator heads'' with lightweight classifiers, we enable models to make early stopping decisions while maintaining performance. 


Our approach challenges existing methods for context efficiency. Previous work show that retrieval-augmented generation (RAG) struggles with multi-hop reasoning and cross-context dependencies \citep{ragvslc}. Meanwhile, compression methods risk information loss through static processing. For instance, the LLMLingua family \citep{llmlingua,longllmlingua,llmlingua2} uses a small language model to filter out unimportant tokens, reducing context based on a fixed compression target. These methods impose predefined compression rates, enforcing a \textit{one-size-fits-all} reduction regardless of content complexity. Similarly, RAG methods predefine a fixed number of top-$k$ retrieved documents. We refer to both RAG and compression-based approaches as \textit{static} methods, in contrast to \textit{dynamic} methods, which do not require predefined compression targets. Our dynamic method preserves the model's native reasoning capabilities – models process the minimal context needed, expanding it only when necessary. This creates a new paradigm where \textit{efficiency emerges naturally from the model's own understanding} rather than external compression heuristics, as demonstrated in Figure \ref{fig:f1}.

 
We validate our approach through comprehensive experiments across six QA datasets (context lengths 0.5K-40K tokens) and three model families (LLaMA, Qwen, Mistral; 1B-70B parameters). We found that LLMs inherently encode context sufficiency signals in specific attention heads (90\% F1 detection). Notably, our method reveals behaviors that aligns well with the scaling behavior of modern LLMs: while smaller models (1B-8B parameters) require explicit sufficiency detection to achieve competitive efficiency, larger models (14B+) exhibit emergent self-assessment capabilities through simple prompting. Our method achieves $1.33\times$ average token reduction with 1.3\% accuracy improvement, while outperforming existing both RAG and the state of the art compression methods. 




==> sections/methods.tex <==
\section{Methodology}  
\label{sec:method}

\noindent\begin{minipage}[t]{0.48\textwidth}
We propose dynamic context cutoff, a method that enables LLMs to identify and process only the minimal sufficient context required for a given task. Our approach leverages internal model activations to detect when enough information has been gathered, reducing token processing while maintaining performance. As illustrated in Figure \ref{fig:method_overview}.

\subsection{Problem Formulation}
Let \(\mathcal{M}\) denote a pre-trained language model. Given an input textual context \(\mathbf{C}\), we process \(\mathbf{C}\) sequentially from left to right by partitioning it into an ordered sequence of chunks \(\{\mathfrak{s}_j\}_{j=1}^m\), where each chunk \(\mathfrak{s}_j\) comprises a contiguous subset of \(\mathbf{C}\) (e.g., a sentence or a fixed percentage of the total tokens). These chunks form a non-overlapping covering of \(\mathbf{C}\), meaning:
\[
\mathlarger{\mathlarger{\mathlarger{\mathbin\Vert}}}_{j=1}^{m} \mathfrak{s}_j = \mathbf{C}, \quad \mathfrak{s}_i \cap \mathfrak{s}_j = \emptyset \text{ for } i \neq j
\]
where \(\mathbin\Vert\) denotes concatenation. We define a sequence of cumulative contexts \(\{\mathbf{C}_i\}_{i=1}^m\), where each cumulative context \(\mathbf{C}_i\) consists of all chunks up to and including the \(i\)-th chunk: 
\[
\mathbf{C}_i = \mathfrak{s}_1 \mathbin\Vert \mathfrak{s}_2 \mathbin\Vert \dots \mathbin\Vert \mathfrak{s}_i, \quad 1 \leq i \leq m
\]
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{-5mm}
\includegraphics[width=\linewidth]{figures/f2.pdf}
\vspace{-6mm}
\captionof{figure}{Our dynamic context cutoff method leverages the model's internal representations to identify when sufficient information has been processed. A lightweight classifier is trained on selected attention heads to detect context sufficiency, leading to token savings while maintaining task performance.
}
\label{fig:method_overview}
\end{minipage}

By construction, these cumulative contexts satisfy the nested proper subset relationship: $\mathbf{C}_1 \subset \mathbf{C}_2 \subset \dots \subset \mathbf{C}_m = \mathbf{C}.$ Given a query \(q\), the goal is to identify the smallest prefix \(\mathbf{C}_k\) (where \(k \leq m\)) such that:
\[
\mathcal{M}(q, \mathbf{C}_k) \approx \mathcal{M}(q, \mathbf{C}).
\]


Let \(\mathcal{M}\) denote a pre-trained language model. Given an input textual context \(\mathbf{C}\), we process \(\mathbf{C}\) sequentially from left to right by partitioning it into an ordered sequence of chunks \(\{\mathfrak{s}_j\}_{j=1}^m\), where each chunk \(\mathfrak{s}_j\) comprises a contiguous subset of \(\mathbf{C}\) (e.g., a sentence or a fixed percentage of the total tokens). These chunks form a non-overlapping covering of \(\mathbf{C}\), meaning:
\[
\mathlarger{\mathlarger{\mathlarger{\mathbin\Vert}}}_{j=1}^{m} \mathfrak{s}_j = \mathbf{C}, \quad \mathfrak{s}_i \cap \mathfrak{s}_j = \emptyset \text{ for } i \neq j
\]
where \(\mathbin\Vert\) denotes concatenation. We define a sequence of cumulative contexts \(\{\mathbf{C}_i\}_{i=1}^m\), where each cumulative context \(\mathbf{C}_i\) consists of all chunks up to and including the \(i\)-th chunk: 
\[
\mathbf{C}_i = \mathfrak{s}_1 \mathbin\Vert \mathfrak{s}_2 \mathbin\Vert \dots \mathbin\Vert \mathfrak{s}_i, \quad 1 \leq i \leq m
\]
By construction, these cumulative contexts satisfy the nested proper subset relationship: $\mathbf{C}_1 \subset \mathbf{C}_2 \subset \dots \subset \mathbf{C}_m = \mathbf{C}.$ Given a query \(q\), the goal is to identify the smallest prefix \(\mathbf{C}_k\) (where \(k \leq m\)) such that:
\[
\mathcal{M}(q, \mathbf{C}_k) \approx \mathcal{M}(q, \mathbf{C}).
\]
Here, \(\mathbf{C}_k\) represents the minimal sufficient context required for the model to answer \(q\) with comparable performance to using the full context \(\mathbf{C}\).

At each step \(i\), a sufficiency classifier \(\mathcal{S}\) iteratively checks whether the current cumulative context \(\mathbf{C}_i\) contains enough information, by comparing its confidence \(\mathcal{S}_c(C_i)\) with a threshold \(\tau\). Formally,
\[
\mathcal{S}(\mathbf{C}_i) = 
\begin{cases} 
1 & \text{if } \mathcal{S}_c(\mathbf{C}_i) \geq \tau  \\
0 & \text{otherwise}
\end{cases},
\]
where \(\mathcal{S}_c: \mathbb{R}^d \rightarrow [0,1]\) is the sufficiency confidence score function, and \(\tau\) is a predefined threshold. If \(\mathcal{S}(\mathbf{C}_i) = 1\), processing terminates, and \(\mathbf{C}_i\) is selected as the minimal sufficient context \(\mathbf{C}_k\). The remaining chunks \(\{\mathfrak{s}_{i+1}, \mathfrak{s}_{i+2}, \ldots, \mathfrak{s}_m\} = \mathbf{C} \setminus \mathbf{C}_k\) are ignored. 

We formulate the problem as early cutoff rather than \textit{searching for an optimal chunk or selecting an arbitrary subset of context}, as is common in RAG methods. This is because that LLMs process text from left to right anyways, so we can reuse the precomputed cache from previous chunks. As opposed to RAG, this allows a contextual understanding of the chunk to determine information sufficiency.


\subsection{Probing for ``Context Sufficiency''}
\label{sec:probing_sufficiency}

We are interested in understanding how context sufficiency is represented within the model and how it can be leveraged to improve efficiency. We probe its intermediate activations. Following prior work on neural network interpretability \citep{iti,deng2024language}, we assess whether certain attention heads encode information predictive of sufficiency. 
The data for probing consists of input cumulative contexts \(\{\mathbf{C}_i\}_{i=1}^n\), each labeled as either sufficient (\(y = 1\)) or insufficient (\(y = 0\)). 

\noindent\begin{minipage}[t]{0.48\textwidth}

For each \(\mathbf{C}_i\), the model produces attention head activations \(\{x_l^h\}\), where \(x_l^h \in \mathbb{R}^D\) is the activation of the \(h\)-th head in the \(l\)-th layer. We train a lightweight binary classifier \(p_\theta(x_l^h)\) on these activations to predict sufficiency:
$p_\theta(x_l^h) = \sigma(\langle \theta, x_l^h \rangle),$ where \(\theta \in \mathbb{R}^D\) are the parameters of the probe, and \(\sigma\) denotes the sigmoid function. The dataset is split into training and validation sets (4:1 ratio) per task. Each classifier's validation F1 score determines the predictive ability of the corresponding head. This selection process is performed only once for all tasks. We discuss more details about the data used probe in \sref{sec:data}.

Figure~\ref{fig:head_acc_sufficiency} shows the F1 scores of probes for all attention heads in LLaMA3.2-1B. A subset of heads, primarily in middle layers, exhibit significantly higher predictive performance. However, depending on different model's architecture, the performance of the probes may vary.
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{-2mm}
\includegraphics[width=\linewidth]{figures/head_heatmap_1b.png}
\vspace{-3mm}
\captionof{figure}{Validation F1 scores for linear probes across all attention heads in LLaMA3.2-1B, sorted row-wise by F1. Darker blue represents higher F1 scores. Some heads show significantly higher performance. More visualizations can be found in \Cref{app:probe}.}
\label{fig:head_acc_sufficiency}
\end{minipage}

These results suggest that the model's internal representations encode latent information about context sufficiency. We leverage this insight to identify the most informative attention heads for further processing.


\subsection{Dynamic Context Cutoff}
\paragraph{Sufficiency Classification}
After identifying the top heads from the probing step, we train multiple lightweight base classifiers \(\{\mathcal{S}_1, \mathcal{S}_2, \ldots, \mathcal{S}_e\}\) on these heads to form an ensemble. The ensemble is constructed using StratifiedKFold with $n=5$ folds, with the best performing models selected based on their mean cross-validation AUC scores to form the final weighted ensemble:

\[
\mathcal{S}_{\text{ensemble}}(\mathbf{C}_i) = \frac{1}{e} \sum_{j=1}^e \mathcal{S}_j(\mathbf{C}_i).
\]
More details in classifier can be found in \Cref{app:details:classifier}. 

\paragraph{Inference with Iterative Forward Passes}
During inference, the full context is processed incrementally as a sequence of nested \(\{\mathbf{C}_i\}_{i=1}^n\), where each \(\{\mathbf{C}_i\}\) contains all preceding tokens. These progressively expanding subsets are passed through the model to extract activations at each step. Next, the ensemble classifier \(\mathcal{S}_{\text{ensemble}}\) predicts whether the current context \(\{\mathbf{C}_i\}_{i=1}^n\) is sufficient.

The activations of all processed chunks are cached to avoid redundant computation. Let \(\mathbf{A}_{\text{cache}}^{i}\) denote cached activations for \(\mathbf{C}_i\), containing the activations of all previous chunks by construction. Activations for the current \(\mathbf{C}_i\) are computed as:
\[\mathbf{A}(\mathbf{C}_i) = f_{\text{model}}(\mathbf{C}_i \setminus \mathbf{C}_{i-1}, \mathbf{A}_{\text{cache}}^{i-1}),\]
where \(f_{\text{model}}\) is the model's forward pass function conditioned on the cached activations \(\mathbf{A}_{\text{cache}}\). 
The iterative process continues until a sufficient context $\mathbf{C}_k$ is identified, as determined by \(\mathcal{S}_{\text{ensemble}}\). If no $\mathbf{C}_i$ is deemed sufficient, the entire input context is processed. In either cases, the cached activations will be reused for generation. The final output is computed as:
\[
\mathcal{M}(\mathbf{C}_k) = \mathcal{M}(\mathbf{C}_k \setminus C_{k-1}, \mathbf{A}_{\text{cache}}^{k-1}).
\]
% The algorithm pseudocode can be found in \Cref{app:algo}.

\paragraph{Alternative Sufficiency Detection}
\label{sec:self_prompt}
As an alternative to classifier-based approach, larger LLMs can leverage their own reasoning capabilities through self-prompting. For each cumulative context $\mathbf{C}_i$, we append a meta-prompt asking the model to evaluate whether it has sufficient information to answer query $q$. The prompt can be found in \Cref{app:prompt}. The model's binary response determines sufficiency, enabling dynamic cutoff without classifiers. In \sref{sec:short_results}, we show that self-prompting becomes increasingly reliable with larger model sizes (14B+ parameters), suggesting sufficiency detection emerges as a capability with scale.





==> sections/related_work.tex <==
\section*{Related Work}
\label{sec:related_work}
\paragraph{Context Efficiency in LLMs.} Transformer-based LLMs initially faced fundamental limitations from fixed context windows \citep{vaswani2017attention}, but recent architectural advances enable processing hundreds of thousands of tokens \citep{jin2024llm,reid2024gemini,llama3.1modelcard,deepseekr1}. However, longer contexts exacerbate computational inefficiencies and performance degradation, where critical information becomes obscured by irrelevant details—a phenomenon termed the ``lost-in-the-middle'' problem \citep{lostinmiddle,RULER}. 
Many context compression methods have been proposed to address this problem \citep{llmlingua,longllmlingua,llmlingua2,icformer,li2024500xcompressor} by predefining a compression rate target and leverage external LLM to filter tokens  or reordering documents. However, these approaches risk discarding task-critical information by prioritizing size reduction over contextual relevance. In contrast, our method dynamically determines sufficiency during processing through the model's internal signals, eliminating rigid compression targets.

\paragraph{Latent Knowledge in Model Activations.} LLMs encode task-relevant knowledge within intermediate activations, often more accurately than their final surface outputs \citep{saunders2022self,iti}. This latent knowledge enables high-quality knowledge graph construction without supervision \citep{wang2020language}, demonstrating its potential for informed decision-making. We extend this insight by probing activation subspaces to detect context sufficiency dynamically. Our approach uniquely identifies when the model has internally synthesized adequate information, mirroring human-like selective processing while reducing computational overhead. This differs fundamentally from static compression methods by leveraging the model's inherent information integration capabilities rather than predefined external heuristics.

